Generalisable Agents for Neural Network Optimisation

Optimising deep neural networks is a challenging task due to complex training dynamics, high computational requirements, and long training times. To address this difficulty, we propose the framework of Generalisable Agents for Neural Network Optimisation (GANNO) -- a multi-agent reinforcement learning (MARL) approach that learns to improve neural network optimisation by dynamically and responsively scheduling hyperparameters during training. GANNO utilises an agent per layer that observes localised network dynamics and accordingly takes actions to adjust these dynamics at a layerwise level to collectively improve global performance. In this paper, we use GANNO to control the layerwise learning rate and show that the framework can yield useful and responsive schedules that are competitive with handcrafted heuristics. Furthermore, GANNO is shown to perform robustly across a wide variety of unseen initial conditions, and can successfully generalise to harder problems than it was trained on. Our work presents an overview of the opportunities that this paradigm offers for training neural networks, along with key challenges that remain to be overcome.

==> content/tables/table_taxonomy.tex <==
\begin{tabular}{cccccc}
  \toprule
 Category & Train = Eval & IID  & OOD  & \multicolumn{2}{c}{Example} \\
 & & $P_{TRAIN} (\cdot) = P_{EVAL} (\cdot)$ & $P_{TRAIN} (\cdot) \neq P_{EVAL} (\cdot)$ & Train& Eval \\ 
 \midrule
  &  &  &  & 3 Layer CNN, & 3 Layer CNN, \\
 1 & $f_\theta, \phi, L$ & $D$ & - & Cifar10 w/o test set, & Cifar10 w/ test set, \\
  &  &  &  & Adam, Cross-Entropy & Adam, Cross-Entropy \\
 %\cline{5-6}
 \noalign{\smallskip}
 & & &  & 3 Layer CNN, & 3 Layer CNN, \\
 2 & $f_\theta, \phi, L$ & - & $D$  & Fashion MNIST, & Cifar10, \\
  &  &  &  & Adam, Cross-Entropy & Adam, Cross-Entropy \\
 %\cline{5-6}
\noalign{\smallskip}
 & & & & 3 Layer CNN, & 5 Layer CNN, \\
 3 & $\phi, L$ & $f_\theta$ & $D$  & Fashion MNIST, & Cifar10, \\
  &  &  &  & Adam, Cross-Entropy & Adam, Cross-Entropy \\
 %\cline{5-6}
 \noalign{\smallskip}
 & & & & 3 Layer CNN, & 5 Layer CNN, \\
 4 & $L$ & $f_\theta$ & $\phi,D$  & Fashion MNIST, & Cifar10, \\
  &  &  &  & SGD, Cross-Entropy & Adam, Cross-Entropy \\
 %\cline{5-6}
 \noalign{\smallskip}
 & & & & 3 Layer CNN, & Vision Transformer, \\
 5 & $L$ & - & $\phi,D,f_\theta$  & Fashion MNIST, & Cifar10, \\
  &  &  &  & SGD, Cross-Entropy & Adam, Cross-Entropy \\
 %\cline{5-6}
 \noalign{\smallskip}
 & & & & 3 Layer CNN, & Vision Transformer, \\
 6 & - & - & $\phi,D,f_\theta,L$  & Fashion MNIST, & Satellite images, \\
  &  &  &  & SGD, Cross-Entropy & Adam, MSE \\
 \bottomrule
\end{tabular}


